Keep It in Mind: User Centric Continual Spatial Intelligence Reasoning in Egocentric Video Streams

We introduce UCS-Bench, a dataset spanning 170+ hours of egocentric visual observations with 8.1K+ timestamped questions for diagnosing User-Centric Continual Spatial intelligence in egocentric video streams. UCS-Bench targets a new problem that emphasizes dynamic spatial reasoning, long-term memory, and their alignment with users' real-time locations. We propose DirectMe, a framework that incrementally constructs and maintains a structured spatial memory from streaming egocentric observations. DirectMe enables robust tracking and recall of object locations, all relative to the user's movement over time. By tightly coupling visual perception with memory updates and spatial reasoning, our approach supports long-horizon queries that require recalling interactions, resolving viewpoint-induced ambiguities, and adapting to dynamic scenes. Our experiments show that DirectMe significantly improves the spatial reasoning of leading multimodal LLMs; it also surpasses many spatially aware and long-form streaming video models. We hope our benchmark and solution will advance spatial intelligence research for egocentric AI assistants. Data and code are available at https://github.com/cocowy1/UCS-Bench.

==> table/compare-instruction-thinking.tex <==
\begin{table*}[htbp] % 如果是双栏排版，建议使用 table* 让表格跨双栏；如果是单栏，用 table 即可
\caption{Comparison of Qwen3-VL instruct and thinking models}
\label{tab:instruct_vs_thinking}
\centering
\vspace{-0.3cm}
\renewcommand{\arraystretch}{1.25} % 增加行高，更美观
\setlength{\tabcolsep}{3pt}        % 减小列间距，防止过宽

\resizebox{1.0\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc|c}
\hline
\multirow{2}{*}{\textbf{Model}}
& \multicolumn{3}{c|}{\textbf{Trajectory \& Movement}}
& \multicolumn{3}{c|}{\textbf{Position \& Orientation}}
& \multicolumn{3}{c|}{\textbf{Proximity \& Reachability}}
& \multicolumn{3}{c|}{\textbf{Category \& Quantity}}
& \multirow{2}{*}{\textbf{Overall}} \\ 
\cline{2-13}
& Overall & My Traj. & Obj. Traj.
& Overall & Ego-centric & Relative
& Overall & Distance & Reachability
& Overall & Obj. Category & Obj. Quantity & \\
\hline
Qwen3-VL-8B-Instruction
& 45.5 & 44.1 & 49.8
& 41.2 & 44.8 & 38.8
& 51.8 & 50.2 & 53.1
& 43.7 & 53.8 & 39.4
& 45.0 \\
Qwen3-VL-8B-Thinking
& 43.0 & 42.4 & 44.8
& 38.4 & 39.3 & 37.9
& 53.6 & 52.9 & 54.2
& 40.5 & 50.9 & 36.0
& 43.0 \\

\hline
\end{tabular}
} % resizebox 结束

\end{table*}


Under a unified configuration of (512 $\times$ 512) resolution and 64-frame input, we compared the performance of the instruction and thinking versions of Qwen3-VL on our benchmark.

Although the thinking model generates richer intermediate processes via long-chain reasoning, its overall score 43.0 is slightly lower than that of the instruction model 45.0. This counter-intuitive phenomenon may stem from the error accumulation effect within the reasoning path. When processing long-sequence video frames, complex reasoning steps might amplify minor perceptual deviations in object trajectories, leading to biased final judgments.


Furthermore, the significant decline of the thinking model in the "Recall \& Quantity" dimension 40.5 vs. 43.7 suggests that lengthy generation processes may induce hallucinations regarding spatial entities or cause attention drift away from the original counting task. 
However, the thinking model excels in the Proximity \& Reachability dimension 53.6, implying that deep reasoning holds a potential advantage for handling distance proximity. 
This performance trade-off reveals that in real-time dynamic spatial perception tasks, excessive reasoning may not be the optimal strategy, maintaining a balance between perceptual intuition and logical deduction is crucial.




% & 43.1 & 43.0 & 44.8
% & 38.2 & 38.5 & 37.9
% & 53.4 & 53.7 & 54.2
% & 45.7 & 40.6 & 36.0
% & 43.0 \\ 

% \begin{table}[htbp]
% \centering
% \begin{tabular}{l|ccc|ccc|ccc|ccc|c}
% \hline
% \multirow{2}{*}{\textbf{Model}}
% & \multicolumn{3}{c|}{\textbf{Trajectory \& Movement}}
% & \multicolumn{3}{c|}{\textbf{Position \& Orientation}}
% & \multicolumn{3}{c|}{\textbf{Proximity \& Reachability}}
% & \multicolumn{3}{c|}{\textbf{Recall \& Quantity}}
% & \multirow{2}{*}{\textbf{Overall}} \\ 
% \cline{2-13}
% & Overall & My Traj. & Obj. Traj.
% & Overall & Position & Orientation
% & Overall & Distance & Reachability
% & Overall & Obj. Recall & Quantity & \\
% \hline
% Qwen3-VL-8B-Instruction
% & 45.5 & 44.1 & 49.8
% & 41.2 & 44.8 & 38.8
% & 51.8 & 50.2 & 53.1
% & 43.7 & 53.8 & 39.4
% & 45.0 \\
% \hline
% Qwen3-VL-8B-Thinking
% & 43.1 & 43.0 & 44.8
% & 38.2 & 38.5 & 37.9
% & 53.4 & 53.7 & 54.2
% & 45.7 & 40.6 & 36.0
% & 22.2 \\ 
% \hline
% \end{tabular}
% \caption{Comparison of Qwen3-VL Instruct and Thinking models}
% \label{tab:instruct_vs_thinking}
% \end{table}






% \begin{table}[htbp]
% \centering
% \begin{tabular}{l|c|c|ccc|ccc|ccc|ccc|c}
% \hline
% \multirow{2}{*}{\textbf{Models}}
% & \multirow{2}{*}{\textbf{Size}}
% & \multirow{2}{*}{\textbf{\# Frame}} 
% & \multicolumn{3}{c|}{\textbf{Trajectory \& Movement}}
% & \multicolumn{3}{c|}{\textbf{Position \& Orientation}}
% & \multicolumn{3}{c|}{\textbf{Proximity \& Reachability}}
% & \multicolumn{3}{c|}{\textbf{Recall \& Quantity}}
% & \multirow{2}{*}{\textbf{Overall}} \\ 
% \cline{4-15}
% & & & Overall & My Traj. & Obj. Traj.
% & Overall & Position & Orientation
% & Overall & Distance & Reachability
% & Overall & Obj. Recall & Quantity & \\
% \hline
% \multirow{2}{*}{Qwen3-VL}
% & \multirow{2}{*}{8B}
% & \multirow{2}{*}{64}
% & 45.5 & 44.1 & 49.8
% & 41.2 & 44.8 & 38.8
% & 51.8 & 50.2 & 53.1
% & 43.7 & 53.8 & 39.4
% & 45.0 \\
% \cline{4-16}
% & &
% & 43.1 & 43.0 & 44.8
% & 38.2 & 38.5 & 37.9
% & 53.4 & 53.7 & 54.2
% & 45.7 & 40.6 & 36.0
% & 22.2 \\ 
% \hline
% \end{tabular}
% \caption{Comparison of Qwen3-VL Instruct and Thinking models}
% \label{tab:instruct_vs_thinking}
% \end{table}


==> table/uniform_evaluation.tex <==

\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{3pt}
\definecolor{lightyellow}{RGB}{255, 250, 194}
% \definecolor{lightred}{RGB}{250, 189, 164}
\definecolor{lightred}{RGB}{253, 158, 158}
\definecolor{lightorange}{RGB}{254, 226, 205}
\begin{table*}[ht]
\footnotesize
\centering
\small
\caption{\textbf{Performance of different models using uniform video sampling on \benchname. }
The \colorbox{lightred}{best}, \colorbox{lightorange}{second-best}, and \colorbox{lightyellow}{third-best} model results are highlighted. Note that \emph{Proximity \& Reachability} is a binary-choice task, while the others are five-way multi-choice. For fair comparison and consistency, all proprietary models are evaluated with up to 50 input images (the maximum supported by the GPT-5 API).}
\vspace{-0.2cm}
\label{tab:uniform_eval}
\resizebox{1.0\textwidth}{!}{
% \begin{tabular}{l| c c | c c c| c c c| c c c| c c c | c}
% \hline
% \multirow{2}{*}{\textbf{Models}} 
% & \multirow{2}{*}{\textbf{Rank}} 
% & \multirow{2}{*}{\textbf{Frame.}} 
% &\multicolumn{3}{c|}{\makecell{\textbf{Embodied trajectory \& Movement Memory}}} 
% &\multicolumn{3}{c|}{\makecell{\textbf{Ego-centric Position \& Orientation Memory}}}
% &\multicolumn{3}{c|}{\makecell{\textbf{Perceived Proximity \& Reachability Memory}}}
% & \multicolumn{3}{c|}{\makecell{\textbf{Object Recall \& Quantity Tracking}}}
% & \multirow{2}{*}{\textbf{Avg.}} 
% \\
% && &  {Avg.} & {My Trajectory}
% & {Object Trajectory} &  {Avg.} & {Ego-centric Position}
% & {Relative Position \& Orientation Memory}&  {Avg.} & {Distance Comparison Memory}
%  & {Reachability Judgment} &  {Avg.}
% &{Object Category Recall}
% & {Quantity Change Tracking}
\begin{tabular}{l| c  c| c c c| c c c| c c c| c c c | c c c|c}
\toprule
\multirow{2}{*}{\textbf{Models}} 
& \multirow{2}{*}{\textbf{Size}} 
& \multirow{2}{*}{\textbf{\# Frame}} 
&\multicolumn{3}{c|}{\makecell{\textbf{Trajectory \& Movement}}} &\multicolumn{3}{c|}{\makecell{\textbf{Position \& Orientation}}}
 &\multicolumn{3}{c|}{\makecell{\textbf{Proximity \& Reachability}}}
& \multicolumn{3}{c|}{\makecell{\textbf{Category \& Quantity}}}
& \multirow{2}{*}{\textbf{Overall}} 
\\
& & &  {Overall} & {My Traj.}
& {Obj. Traj.} &  {Overall} & {Ego-centric}
& {Relative}&  {Overall} & {Distance}
 & {Reachability} &  {Overall}
&{Obj. Category}
& {Obj. Quantity} &

\\
\hline

\textbf{Baseline} & & & & & & & & & & & & & & & \\
Human 
% & -  & -
% & 91.6 & 90.9 & 94.1 
% & 87.8 & 84.0 & 89.8
% & 96.5 & 93.2 & 98.2
% & 90.4 & 94.3 & 89.2 & 91.2\\
% Human Level 
& - & -
& 91.6 & 90.9 & 94.1
& 87.8 & 84.0 & 89.8
& 96.3 & 95.0 & 98.2
& 90.2 & 94.3 & 88.1 & 91.0 \\
Random 
& - & -
& 19.1 & 20.8 & 14.2
& 22.7 & 24.4 & 21.5
& 50.2 & 51.8 & 48.1
& 19.4 & 20.3 & 19.0 & 25.7 \\
% Random Level 
% & 0 & 26.7 & 64
% & 23.1 & 23.4 & 22.1
% & 22.8 & 26.3 & 20.4
% & 44.9 & 40.7 & 48.1
% & 22.1 & 25.5 & 20.6 \\
\hline

\textbf{Proprietary Models / 100B+ Models} & & & & & & & & & & & & & & & \\
Deepseek-V3
& - & 50
& 34.7 & 34.4 & 35.4
& 29.9 & 33.1 & 27.8
& 40.4 & 41.6 & 39.5
& 26.0 & 33.3 & 22.8 & 31.6   \\
GPT-5
& - & 50 
& 44.8 & 43.9 & 47.5 
& 38.2 & 37.2 & 38.8 
& 53.4 & 50.7 & 55.6 
& 41.3 & 55.6 & 35.1 & 43.5     \\
Doubao-seed-1.6V
& - & 50 
& 49.5 & 48.8 & 51.8
& 41.5 & 44.6 & 39.5
& \colorbox{lightred}{54.8} & \colorbox{lightred}{55.2} & 54.5
& 43.3 & 56.4 & 37.7 & 46.4 \\
\hline

\textbf{Open-Source Models / 100B- Models} & & & & & & & & & & & & & & &  \\
\multirow{2}{*}{Qwen2.5-VL}
& 7B & 64
& 44.9 & 45.2 & 44.3
& 39.6 & 42.7 & 37.6
& 51.1 & 46.0 & 55.0
& 45.5 & 53.6 & \colorbox{lightorange}{42.0} & 44.9 \\

& 32B  & 64
& 50.6 & 49.7 & 53.2
& 40.1 & 41.4 & 39.3
& \colorbox{lightyellow}{53.2} & 50.2 & \colorbox{lightyellow}{55.6}
& \colorbox{lightyellow}{47.1} & 58.1 & \colorbox{lightred}{42.3} & 47.2   \\
\multirow{2}{*}{Qwen3-VL}
& 8B & 64
& 45.4 & 44.8 & 47.4
& 41.1 & \colorbox{lightyellow}{46.2} & 37.8
& 51.1 & 49.7 & 52.2
& 46.0 & \colorbox{lightyellow}{58.8} & 40.5 & 45.6 \\

& 32B & 64
& \colorbox{lightyellow}{51.9} & \colorbox{lightorange}{51.0} & \colorbox{lightyellow}{54.4}
& \colorbox{lightorange}{45.5} & \colorbox{lightred}{48.9} & \colorbox{lightyellow}{43.2}
& 51.5 & 48.7 & 53.7
& \colorbox{lightred}{47.9} & \colorbox{lightorange}{61.8} & \colorbox{lightyellow}{41.8} & \colorbox{lightorange}{48.8}   \\
\multirow{2}{*}{Intern3-VL}
& 7B & 64
& 45.7 & 45.7 & 45.7
& 40.0 & 40.1 & 39.9
& 51.9 & 48.9 & 54.3
& 45.2 & 58.4 & 39.5 & 45.2 \\

& 38B & 64
% & 56.08 & 54.4 & 60.9
% & 45.61 & 48.2 & 43.8
% & 52.34 & 52.4 & 52.2
% & 47.64 & 62.7 & 41.1 & 49.91   \\
& \colorbox{lightred}{56.1} & \colorbox{lightred}{54.4} & \colorbox{lightred}{60.9}
& \colorbox{lightred}{45.6} & \colorbox{lightorange}{48.2} & \colorbox{lightorange}{43.8}
& 52.3 & \colorbox{lightyellow}{52.4} & 52.2
& \colorbox{lightorange}{47.6} & \colorbox{lightred}{62.7} & 41.1 & \colorbox{lightred}{49.9}   \\
\multirow{2}{*}{Intern3.5-VL}
& 7B & 64
& 45.0 & 44.1 & 47.9
& 35.2 & 36.6 & 34.3
& 50.1 & 50.4 & 49.9
& 41.7 & 53.7 & 36.5 & 42.4\\

& 38B & 64
& \colorbox{lightorange}{52.0} & \colorbox{lightyellow}{49.8} & \colorbox{lightorange}{58.7}
& \colorbox{lightyellow}{43.9} & 43.7 & \colorbox{lightred}{44.0}
& \colorbox{lightorange}{53.4} & \colorbox{lightorange}{54.0} & 52.9
& 45.3 & 58.0 & 39.8 & \colorbox{lightyellow}{48.0}    \\
LLaVA-Video
& 7B & 64
& 43.2 & 42.6 & 45.0
& 38.6 & 40.2 & 37.5
& 48.2 & 46.7 & 49.4
& 42.2 & 54.2 & 37.0 & 42.6  \\
Intern-Video2.5
& 8B & 64
& 45.5 & 44.5 & 48.4
& 38.1 & 40.7 & 36.4
& 51.1 & 47.6 & 53.8
& 43.5 & 54.7 & 39.0 & 39.7  \\
\hline

\textbf{Spatial Models} & & & & & & & & & & & & & & &  \\
Spatial-MLLM
& 3B & 64
& 34.0 & 34.8 & 31.5
& 26.6 & 30.5 & 24.0
& 48.5 & 43.2 & 52.6
& 32.1 & 38.7 & 29.3 & 34.2  \\
ViLaSR
& 7B & 64
& 40.0 & 40.8 & 37.5
& 32.5 & 34.0 & 31.5
& 51.6 & 45.4 & \colorbox{lightorange}{56.4}
& 40.4 & 48.1 & 37.1 & 40.4 \\
SenseNova-SI
& 8B & 64
% & 38.26 & 39.1 & 35.6
% & 29.43 & 30.0 & 29.0
% & 48.39 & 46.5 & 49.8
% & 35.71 & 43.9 & 32.1 & 37.03  \\
& 38.3 & 39.1 & 35.6
& 29.4 & 30.0 & 29.0
& 48.4 & 46.5 & 49.8
& 35.7 & 43.9 & 32.1 & 37.0 \\
Cambrain
& 7B & 64
% & 45.17 & 45.6 & 43.6
% & 36.51 & 38.1 & 35.4
% & 51.46 & 46.0 & 55.6
% & 42.56 & 52.2 & 38.3 & 43.26   \\
& 45.2 & 45.6 & 43.6
& 36.5 & 38.1 & 35.4
& 51.5 & 46.0 & 55.6
& 42.6 & 52.2 & 38.3 & 43.3   \\
VGLLM
& 8B & 64
% & 32.84 & 33.2 & 31.6
% & 30.73 & 34.2 & 28.4
% & 48.22 & 43.7 & 51.8
% & 33.22 & 43.0 & 29.1 & 32.90 \\
& 32.8 & 33.2 & 31.6
& 30.7 & 34.2 & 28.4
& 48.2 & 43.7 & 51.8
& 33.2 & 43.0 & 29.1 & 32.9 \\
\hline
\textbf{Streaming Models} & & & & & & & & & & & & & & &  \\
Flash-VStream
& 7B & 1 fps
& 25.9 & 27.3 & 21.9
& 22.9 & 24.0 & 22.3
& 48.1 & 44.0 & 51.2
& 23.1 & 26.3 & 21.6 & 28.3 \\
VideoChat-Online
& 4B & 1 fps
& 35.7 & 36.1 & 34.2
& 30.5 & 32.0 & 29.5
& 51.6 & 45.4 & \colorbox{lightred}{56.6}
& 35.6 & 42.3 & 32.7 & 37.3   \\
Dispider
& 7B & 1 fps
& 39.3 & 40.3 & 36.1
& 34.6 & 39.3 & 31.6
& 43.7 & 44.9 & 42.7
& 39.9 & 45.1 & 37.7 & 39.1 \\
% \hline
% \modelname\ (Ours)
% & - & - & -
% & - & - & 
% & - & - & 
% & - & - & 
% & - & - &  \\
\bottomrule
\end{tabular}
}
\end{table*}


% \renewcommand{\arraystretch}{1.25} % 调整行高
% \setlength{\tabcolsep}{3pt} % 调整列间距
% \definecolor{lightyellow}{RGB}{255, 250, 194}
% \definecolor{lightred}{RGB}{250, 189, 164}
% \definecolor{lightorange}{RGB}{254, 226, 205}
% \begin{table*}[ht]
% % \renewcommand\tabcolsep{2pt}
% % \renewcommand\arraystretch{1.2}
% \footnotesize
%     \centering
%     \small
%     \resizebox{1.0\textwidth}{!}{
% \begin{tabular}{l| c c| c c c c| c c c c| c c c c c c| c c c c c| c c c}
% % &  \multicolumn{2}{c|}{Total} & \multicolumn{9}{c|}{Total} & \multicolumn{4}{c|}{Total} & \multicolumn{10}{c}{Total} \\
% % \toprule
%     \textbf{Models} & \rotatebox{75}{\textbf{Rank}} & \normalsize\rotatebox{75}{\textbf{Avg.}} & \normalsize\rotatebox{75}{\makecell{\textbf{Global Perception} \\ \textbf{\& Mapping}}} & 
%     \scriptsize \rotatebox{75}{Scene Layout Reason} & \scriptsize \rotatebox{75}{Panoramic Counting} & \scriptsize \rotatebox{75}{Cognitive Mapping} & \normalsize\rotatebox{75}{\makecell{\textbf{Navigation} \\ \textbf{\& Planning}}} & \scriptsize \rotatebox{75}{Outdoor Navigation} & \scriptsize \rotatebox{75}{Path Planning Logic} & \scriptsize \rotatebox{75}{Ego/Objects-motion Perception} & \normalsize\rotatebox{75}{\makecell{\textbf{Multi-View \&} \\ \textbf{Geometric Reasoning}}} & \scriptsize \rotatebox{75}{Real-world QA} & \scriptsize \rotatebox{75}{View Consistency} & \scriptsize \rotatebox{75}{Perspective Shift} & \scriptsize \rotatebox{75}{Pure Mental Rotation} & \scriptsize \rotatebox{75}{Spatial Puzzles}& \normalsize\rotatebox{75}{\makecell{\textbf{Embodied \&} \\ \textbf{Fine-grained}}} & \scriptsize \rotatebox{75}{Hand-Object Interaction} & \scriptsize \rotatebox{75}{Fine-grained Tracking} & \scriptsize\rotatebox{75}{Depth \& Distance} & \scriptsize \rotatebox{75}{Action Prediction} & \normalsize\rotatebox{75}{\textbf{Logic Detection}} & \scriptsize \rotatebox{75}{Object Peranence} & \scriptsize\rotatebox{75}{Direction Judgement}\\
%     \hline
%     \textbf{Baseline} & & & & & & & & & & & & & & & & & & & & & & & & \\
%     Human Level & 1 & 74.42 & 67.85 & 80.00 & 73.42 & 26.77 & 78.22 & 64.67 & 95.00 & 83.00 & 77.45 & 98.51 & 75.00 & 71.23 & 68.00 & 93.00 & 71.86 & 71.50 & 72.13 & 77.67 & 55.00 & 76.22 & 70.00 & 81.20 \\
%     Random Level & 32 & 27.30 & - & 25.00 & 25.00 & - & 34.72 & 12.50 & 25.00 & 50.00 & 24.99 & 24.96 & 25.00 & 25.00 & 25.00 & 25.00 & 24.98 & 24.95 & 25.00 & 25.00 & 25.00 & 25.00 & 25.00 & 25.00 \\
%     \hline
%     \textbf{Proprietary Models / 100B+ Models} & & & & & & & & & & & & & & & & & & & & & & & & \\
%     GPT-4o~\cite{hurst2024gpt} & 6 & \cellcolor{lightyellow} 45.70 & 17.74 & 11.50 & 26.58 & 3.61 & 53.78 & 32.00 & 85.00 & 60.60 & \cellcolor{lightyellow} 54.55 & 91.85 & 39.00 & 51.28 & 37.00 & 74.00 & \cellcolor{lightyellow} 47.78 & 30.00 & 56.07 & 70.67 & 25.00 & 45.33 & 74.00 & 22.40 \\
%     DeepSeek-V3.2~\cite{liu2025deepseek} & 22 & 37.06 & 19.68 & 13.50 & 29.24 & 3.30 & 49.89 & 19.67 & 87.00 & 60.60 & 46.65 & 93.33 & 38.00 & 33.05 & 36.00 & 72.00 & 33.67 & 29.50 & 39.34 & 38.00 & 20.00 & 25.11 & 21.50 & 28.00 \\
%     % ~~~-thinking & - & 38.98 & 22.14 & 17.5 & 32.23 & 1.04 & 47 & 21.33 & 77 & 56.4 & 40.43 & 93.33 & 30 & 27.92 & 23 & 62 & 38.1 & 36.25 & 48.52 & 30.33 & 37 & 44.89 & 57 & 35.2 \\
%     ~~~-thinking & 10 & 43.74 & \cellcolor{lightyellow} 22.02 & 16.50 & 32.89 & 0.33 & \cellcolor{lightyellow} 61.22 & 12.00 & 86.00 & 85.80 & 53.71 & 97.78 & 37.00 & 47.29 & 37.00 & 80.00 & 32.76 & 13.25 & 55.08 & 37.33 & 29.00 & \cellcolor{lightyellow} 46.22 & 63.00 & 32.80\\
%     % Claude-4-Sonnet & - & & & & & & & & & & & & & & & & & & & & & & & \\
%     % Gemini-3-Flash~\cite{gemini3flash} & - & & & & & & & & & & & & & & & & & & & & & & & \\
%     % Gemini-3-Pro & - & & & & & & & & & & & & & & & & & & & & & & & \\
%     Gemini-3-Flash-preview~\cite{gemini3flash} & 2 & \cellcolor{lightred} 59.46 & \cellcolor{lightred} 35.66 & 44.50 & 38.87 & 8.34 & \cellcolor{lightred} 77.11 & 47.00 & 89.00 & 92.80 & \cellcolor{lightred} 68.54 & 96.30 & 50.50 & 72.65 & 45.00 & 84.00 & \cellcolor{lightred} 51.31 & 27.75 & 65.25 & 76.67 & 27.00 & \cellcolor{lightred} 59.11 & 61.00 & 57.60 \\
%     \hline
%     \textbf{Open-Source Models / 100B- Models} & & & & & & & & & & & & & & & & & & & & & & & & \\
%     LlaVA-1.5-7B~\cite{liu2024improved} & 31 & 30.53 & \cellcolor{lightred} 29.18 & 28.00 & 39.53 & 0.34 & 39.33 & 16.33 & 95.00 & 42.00 & 29.78 & 28.89 & 31.00 & 31.91 & 25.00 & 22.00 & 25.52 & 23.25 & 30.16 & 22.33 & 30.00 & 28.44 & 22.50 & 33.20 \\
%     % Llama-3-8B & - & 34.01 & 14.44 & 20.5 & 14.62 & 1.77 & 43.78 & 15.33 & 73 & 55 & 44.02 & 87.41 & 29 & 40.17 & 35 & 32 & 32.85 & 29.5 & 33.44 & 38.33 & 28 & 24.89 & 25.5 & 24.4 \\
%     Llama-3.1-8B~\cite{grattafiori2024llama} & 27 & 34.78 & 14.28 & 15.00 & 17.94 & 1.82 & 45.11 & 17.00 & 71.00 & 56.80 & 36.60 & 88.15 & 31.50 & 21.94 & 27.00 & 40.00 & 39.73 & 51.75 & 34.43 & 31.33 & 33.00 & 26.00 & 19.50 & 31.20 \\
%     InternVL3-2B~\cite{zhu2025internvl3} & 29 & 33.92 & 20.68 & 16.50 & 29.90 & 1.28 & 42.67 & 18.00 & 87.00 & 48.60 & 39.59 & 87.41 & 32.00 & 30.48 & 24.00 & 36.00 & 31.22 & 6.75 & 36.39 & 24.67 & 13.00 & 30.22 & 22.50 & 36.40 \\
%     InternVL3-8B~\cite{zhu2025internvl3} & 20 & 38.42 & 22.68 & 13.50 & 35.88 & 1.29 & 35.00 & 10.33 & 71.00 & 42.60 & 46.41 & 93.33 & 33.50 & 38.18 & 27.00 & 68.00 & 47.06 & 53.75 & 46.56 & 43.33 & 33.00 & 30.22 & 29.00 & 31.20 \\
%     % InternVL3-14B & - & 42.58 & 20.19 & 11 & 31.89 & 3.32 & 48.89 & 20.67 & 89 & 57.8 & 45.69 & 97.04 & 35 & 33.05 & 30 & 70 & 49.59 & 45.5 & 51.15 & 59.33 & 32 & 36.89 & 41 & 33.6 \\
%     % InternVL3\_5-2B & - & 34.75 & 24.19 & 11 & 39.87 & 3.38 & 45.56 & 13.67 & 88 & 56.2 & 41.87 & 87.41 & 39 & 32.19 & 23 & 36 & 30.68 & 32 & 35.74 & 27.67 & 19 & 24 & 17.5 & 29.2 \\
%     InternVL3.5-4B~\cite{wang2025internvl3} & 17 & 39.95 & 25.79 & 15.00 & 40.20 & 4.01 & 47.44 & 17.67 & 88.00 & 57.20 & 44.50 & 95.56 & 35.50 & 32.48 & 28.00 & 60.00 & 38.73 & 36.50 & 43.93 & 38.00 & 34.00 & 38.44 & 46.50 & 32.00 \\
%     % \rowcolor{lightgray}
%     ~~~-thinking & 18 & 38.98 & 22.14 & 17.50 & 32.23 & 1.04 & 47.00 & 21.33 & 77.00 & 56.40 & 40.43 & 93.33 & 30.00 & 27.92 & 23.00 & 62.00 & 38.10 & 36.25 & 48.52 & 30.33 & 37.00 & 44.89 & 57.00 & 35.20 \\
%     InternVL3.5-8B~\cite{wang2025internvl3} & 12 & 43.27 & 26.14 & 18.50 & 38.87 & 3.09 & 49.78 & 19.33 & 90.00 & 60.00 & 44.26 & 94.81 & 34.50 & 33.05 & 26.00 & 62.00 & 48.78 & 48.00 & 52.46 & 49.33 & 39.00 & 37.78 & 45.50 & 31.60 \\
%     % \rowcolor{lightgray}
%     ~~~-thinking & 4 & \cellcolor{lightyellow} 46.43 & 18.65 & 14.50 & 27.24 & 1.07 & \cellcolor{lightyellow} 62.00 & 24.33 & 85.00 & 80.00 & 52.87 & 96.30 & 39.00 & 46.72 & 28.00 & 84.00 & 45.61 & 42.75 & 57.05 & 44.00 & 27.00 & 42.44 & 52.50 & 34.40 \\
%     % InternVL3\_5-14B-Instruct & - & 41.47 & 23.64 & 16.5 & 35.55 & 2.05 & 49.33 & 23.67 & 88 & 57 & 46.17 & 95.56 & 35 & 34.47 & 34 & 64 & 42.81 & 34 & 47.54 & 56 & 24 & 37.56 & 44 & 32.4 \\
%     % InternVL3\_5-30B-A3B & - & 40.98 & 20.32 & 12.5 & 30.23 & 6.12 & 47.44 & 19 & 88 & 56.4 & 53.59 & 97.04 & 36.5 & 50.43 & 31 & 72 & 40.54 & 33.5 & 41.31 & 49 & 41 & 33.33 & 30 & 36 \\
%     Qwen2.5-3B~\cite{yang2024qwen2} & 26 & 34.81 & \cellcolor{lightyellow} 27.93 & 19.50 & 42.52 & 0.83 & 45.44 & 15.67 & 75.00 & 57.40 & 35.05 & 83.70 & 32.50 & 19.66 & 32.00 & 28.00 & 32.85 & 29.25 & 38.03 & 36.00 & 22.00 & 27.11 & 18.00 & 34.40 \\
%     % Qwen2.5-7B & - & 36.43 & 12.77 & 16 & 14.62 & 0.77 & 41.22 & 15.67 & 84 & 48 & 45.81 & 85.93 & 32 & 46.44 & 22 & 36 & 40.36 & 43.75 & 40.66 & 38.67 & 31 & 31.33 & 27.5 & 34.4 \\
%     Qwen2.5-72B~\cite{yang2024qwen2} & 13 & 42.57 & 14.28 & 15.00 & 17.94 & 1.84 & 50.56 & 26.33 & 90.00 & 57.20 & 53.23 & 95.56 & 39.50 & 48.43 & 35.00 & 64.00 & 47.15 & 36.75 & 43.61 & 70.00 & 31.00 & 33.33 & 32.00 & 34.40 \\
%     Qwen2.5-VL-3B~\cite{bai2025qwen2} & 25 & 35.54 & 21.49 & 10.00 & 35.22 & 3.17 & 40.89 & 11.33 & 79.00 & 51.00 & 40.55 & 91.85 & 36.50 & 27.07 & 27.00 & 40.00 & 39.10 & 48.00 & 33.44 & 34.00 & 36.00 & 25.56 & 18.00 & 31.60 \\
%     % Qwen2.5-VL-7B & - & 34.7 & 19.9 & 15.5 & 27.57 & 5.61 & 42.78 & 15 & 62 & 55.6 & 46.29 & 94.81 & 35 & 37.32 & 29 & 58 & 32.67 & 23.5 & 43.61 & 37.33 & 22 & 21.78 & 28.5 & 16.4 \\
%     Qwen2.5-VL-72B~\cite{bai2025qwen2} & 8 & 45.45 & 19.29 & 13.00 & 28.90 & 2.94 & 55.67 & 33.33 & 89.00 & 62.40 & \cellcolor{lightyellow} 53.47 & 95.56 & 36.50 & 48.43 & 38.00 & 74.00 & \cellcolor{lightyellow} 49.59 & 33.00 & 52.79 & 76.00 & 27.00 & 34.89 & 47.50 & 24.80 \\
%     % Qwen3-4B-Instruct-2507 & - & 36.59 & 18.95 & 14 & 27.91 & 1.91 & 44.22 & 16.67 & 69 & 55.8 & 40.91 & 89.63 & 34 & 28.77 & 23 & 58 & 38.1 & 47.75 & 34.43 & 32 & 29 & 33.11 & 30.5 & 35.2 \\
%     % Qwen3-30B-A3B-Instruct-2507 & - & 36.5 & 18.38 & 16.5 & 24.92 & 2.49 & 42 & 15.67 & 92 & 47.8 & 46.41 & 92.59 & 37 & 35.9 & 32 & 62 & 37.38 & 33.75 & 36.39 & 41 & 44 & 29.11 & 20.5 & 36 \\
%     Qwen3-4B~\cite{yang2024qwen2} & 28 & 34.68 & 12.44 & 16.00 & 13.29 & 2.76 &  45.89 & 20.33 & 84.00 & 53.60 & 43.06 & 87.41 & 37.50 & 34.76 & 25.00 & 40.00 & 34.57 & 38.25 & 36.07 & 29.67 & 30.00 & 26.67 & 20.00 & 32.00 \\
%     % \rowcolor{lightgray}
%     ~~~-thinking & 14 & 42.26 & 17.24 & 13.00 & 25.25 & 1.62 & 52.67 & 22.67 & 75.00 & 66.20 & \cellcolor{lightyellow} 53.47 & 91.11 & 41.00 & 50.71 & 25.00 & 78.00 & 39.73 & 33.50 & 44.59 & 48.00 & 25.00 & 40.22 & 48.50 & 33.60 \\
%     Qwen3-8B~\cite{yang2024qwen2} & 21 & 37.91 & 18.20 & 14.00 & 26.58 & 1.40 & 45.11 & 19.33 & 66.00 & 56.40 & 41.87 & 91.11 & 32.00 & 31.62 & 24.00 & 56.00 & 42.99 & 43.75 & 37.70 & 48.67 & 39.00 & 30.00 & 26.50 & 32.80 \\
%     % \rowcolor{lightgray}
%     ~~~-thinking & 9 & 45.04 & 17.49 & 13.50 & 25.58 & 1.13 & 58.78 & 22.00 & 72.00 & 78.20 & 52.51 & 94.07 & 34.50 & 49.57 & 27.00 & 84.00 & 44.16 & 39.75 & 47.87 & 51.67 & 28.00 & 42.67 & 48.00 & 38.40 \\
    
%     Qwen3-VL-4B~\cite{bai2025qwen2} & 19 & 38.67 & 18.81 & 12.50 & 28.57 & 2.04 & 47.44 & 17.00 & 86.00 & 58.00 & 45.81 & 94.07 & 34.50 & 37.32 & 26.00 & 60.00 & 38.19 & 37.00 & 37.38 & 42.00 & 34.00 & 35.56 & 34.00 & 36.80 \\
%     ~~~-thinking & 11 & 43.70 & 15.81 & 15.50 & 21.26 & 0.00 & 58.00 & 22.00 & 80.00 & 75.20 & 51.79 & 92.59 & 37.50 & 46.72 & 28.00 & 82.00 & 39.91 & 29.00 & 44.26 & 55.67 & 23.00 & \cellcolor{lightyellow} 46.67 & 54.00 & 40.80 \\
%     Qwen3-VL-8B~\cite{bai2025qwen2} & 16 & 42.10 & 25.74 & 11.50 & 43.52 & 0.69 & 45.78 & 20.67 & 81.00 & 53.80 & 48.44 & 92.59 & 28.50 & 47.01 & 24.00 & 68.00 & 43.53 & 41.75 & 43.28 & 51.00 & 29.00 & 41.33 & 45.00 & 38.40 \\
%     ~~~-thinking & 7 & 45.66 & 20.97 & 16.00 & 31.23 & 0.00 & 59.11 & 27.00 & 77.00 & 74.80 & 52.99 & 94.81 & 37.50 & 52.14 & 28.00 & 58.00 & 43.62 & 30.50 & 49.84 & 60.00 & 28.00 & 43.11 & 51.50 & 36.40 \\
%     Qwen3-VL-32B~\cite{bai2025qwen2} & 5 & 45.90 & 15.74 & 12.00 & 22.92 & 1.61 & 59.44 & 31.67 & 87.00 & 70.60 & 45.81 & 98.52 & 35.50 & 30.77 & 39.00 & 64.00 & 53.67 & 45.25 & 54.75 & 72.67 & 27.00 & 40.22 & 42.50 & 38.40 \\
%     ~~~-thinking & 3 & \cellcolor{lightred} 51.06 & 16.34 & 13.00 & 23.92 & 0.20 & \cellcolor{lightred} 68.67 & 28.67 & 77.00 & 91.00 & \cellcolor{lightred} 59.45 & 96.30 & 39.00 & 59.54 & 40.00 & 80.00 & \cellcolor{lightred} 49.68 & 33.50 & 58.69 & 69.00 & 29.00 & \cellcolor{lightred} 50.00 & 54.00 & 46.80 \\

%     \hline
%     \textbf{Spatial Models} & & & & & & & & & & & & & & & & & & & & & & & & \\   
%     Space-Qwen-3B~\cite{chen2024spatialvlm} & 33 & 27.26 & 16.35 & 21.00 & 17.28 & 4.24 & 36.33 & 11.33 & 71.00 & 44.40 & 27.75 & 44.44 & 22.50 & 25.64 & 24.00 & 26.00 & 29.77 & 27.00 & 38.36 & 28.85 & 18.00 & 16.22 & 19.00 & 14.00 \\
%     SpaceThinker-3B~\cite{chen2024spatialvlm} & 30 & 33.83 & \cellcolor{lightred} 20.73 & 18.50 & 28.24 & 2.58 & 43.11 & 12.00 & 61.00 & 58.20 & 38.04 & 86.67 & 36.00 & 25.36 & 21.00 & 38.00 & 32.22 & 32.00 & 32.13 & 33.33 & 30.00 & \cellcolor{lightyellow} 28.89 & 16.00 & 39.20 \\
%     Robobrain2.0-7B~\cite{team2025robobrain} & 24 & 35.52 & 18.41 & 16.50 & 25.58 & 0.62 & 36.78 & 17.67 & 67.00 & 42.20 & \cellcolor{lightyellow} 46.17 & 92.59 & 33.50 & 39.32 & 26.00 & 60.00 & \cellcolor{lightyellow} 41.36 & 40.50 & 40.66 & 46.67 & 31.00 & 21.78 & 23.00 & 20.80 \\
%     SpaceR-7B~\cite{ouyang2025spacer} & 23 & \cellcolor{lightyellow} 36.42 & 19.40 & 12.50 & 27.91 & 7.60 & \cellcolor{lightyellow} 44.22 & 13.33 & 72.00 & 57.20 & 43.90 & 93.33 & 36.50 & 29.91 & 33.00 & 60.00 & 37.56 & 37.75 & 44.59 & 32.67 & 30.00 & 26.89 & 31.50 & 23.20 \\
%     Cosmos-Reason2-8B~\cite{azzolini2025cosmos} & 15 & \cellcolor{lightred} 42.13 & \cellcolor{lightyellow} 20.59 & 14.50 & 31.23 & 0.76 & \cellcolor{lightred} 47.89 & 21.00 & 89.00 & 55.80 & \cellcolor{lightred} 50.00 & 92.59 & 33.00 & 49.86 & &  & &  &  &  & & & & \\
%     % \bottomrule
% \end{tabular}
%     }
%     \caption{\textbf{Performance of different models on SiT bench.} The highest and second-highest in each category are highlighted with \colorbox{lightred}{light red} and \colorbox{lightyellow} {light yellow}, respectively.}
%     \label{tab:results_categories}
%     \vspace{-5mm}
% \end{table*}
